Singular General Relativity

This work presents the foundations of Singular Semi-Riemannian Geometry and Singular General Relativity, based on the author's research. An extension of differential geometry and of Einstein's equation to singularities is reported. Singularities of the form studied here allow a smooth extension of the Einstein field equations, including matter. This applies to the Big-Bang singularity of the FLRW solution. It applies to stationary black holes, in appropriate coordinates (since the standard coordinates are singular at singularity, hiding the smoothness of the metric). In these coordinates, charged black holes have the electromagnetic potential regular everywhere. Implications on Penrose's Weyl curvature hypothesis are presented. In addition, these singularities exhibit a (geo)metric dimensional reduction, which might act as a regulator for the quantum fields, including for quantum gravity, in the UV regime. This opens the perspective of perturbative renormalizability of quantum gravity without modifying General Relativity.

==> sections/1112.4508-bb-flrw-abstract.tex <==
We show that the Big Bang singularity of the Friedmann-Lema\^itre-Robertson-Walker model does not raise major problems to General Relativity. We prove a theorem showing that the Einstein equation can be written in a non-singular form, which allows the extension of the spacetime before the Big Bang.

These results follow from 	our research on singular semi-Riemannian geometry and singular General Relativity \cite{Sto11a,Sto11b,Sto11d} (which we applied in previous chapters to the black hole singularities \cite{Sto11e,Sto11f,Sto11g,Sto12e}).


==> sections/1203.1819-bb-flrw-ex-abstract.tex <==
Einstein's equation, in its standard form, breaks down at the Big Bang singularity. We will see here that the expanded Einstein equation remains smooth at the Big Bang singularity of the Friedmann-Lema\^itre-Robertson-Walker model.

==> sections/1203.1819-bb-flrw-ex-body.tex <==
%--------------------------------------------------------
\subsection{Beyond the {\FLRW} Big-Bang singularity}
\label{s_beyond_big_bang}


\begin{theorem}
For the {\FLRW} metric \eqref{eq_flrw_metric},
 with $a: I\to \R$ a smooth function of time, the tensors $R_{abcd}$, $S_{abcd}$, and $E_{abcd}$ are smooth, and consequently the expanded Einstein equation is smooth too, even when $a(t)=0$.
\end{theorem}
\begin{proof}
If we denote by $\widetilde T_{ab}:= \kappa T_{ab} - \Lambda g_{ab}$,
\begin{equation}
\label{eq_flrw_curv_ricci}
\begin{array}{lll}
R_{ab} &=& \widetilde T_{ab} - \dsfrac{1}{2}g^{st}\widetilde T_{st} \\
&=& \kappa T_{ab} - \Lambda g_{ab} - \dsfrac{\kappa}{2} g^{st} T_{st} g_{ab} + 2 \Lambda g_{ab} \\
&=& \kappa\(\rho + \dsfrac{p}{c^2}\) u_a u_b + \kappa p g_{ab} - \dsfrac{\kappa}{2} \(-\rho c^2 - p + 4 p\) g_{ab} + \Lambda g_{ab} \\
&=& \kappa\(\rho + \dsfrac{p}{c^2}\) u_a u_b + \dsfrac{\kappa}{2} \(\rho c^2 - p\) g_{ab} + \Lambda g_{ab} \\
\end{array}
\end{equation}
From equations \eqref{eq_friedmann_density}, \eqref{eq_acceleration}, and \eqref{eq_flrw_curv_ricci}, we can see that the Ricci tensor has the form
\begin{equation}
\label{eq_flrw_curv_ricci_a}
	R_{ab} = a^{-2}(t)\alpha(t) u_a u_b + a^{-2}(t)\beta(t) g_{ab}.
\end{equation}
where $\alpha(t)$ and $\beta(t)$ are smooth functions.
Similarly,
\begin{equation}
\label{eq_flrw_curv_scalar}
\begin{array}{lll}
R &=& g^{st}R_{st} \\
&=& \kappa\(-\rho c^2 - p + 2 \rho c^2 - 2 p\) + 4\Lambda \\
&=& \kappa\(\rho c^2 - 3p\) + 4\Lambda \\
\end{array}
\end{equation}
and there is a smooth function $\gamma(t)$ so that
\begin{equation}
\label{eq_flrw_curv_scalar_a}
R = a^{-2}(t)\gamma(t).
\end{equation}

We need to check that $a^{-2}(t)$ is compensated in $S_{abcd}$ and $E_{abcd}$, so that $a(t)$ appears to a non-negative power.

Since the {\FLRW} metric \eqref{eq_flrw_metric} is diagonal in the standard coordinates, each term in $(g\circ g)_{abcd}$ is of the form $g_{aa}g_{bb}$, with $a\neq b$. This means that at least $a\neq t$ or $b\neq t$ holds, and from \eqref{eq_flrw_metric} we conclude that $g_{aa}g_{bb}$ contains $a(t)$ at least to the power $2$. Therefore, the scalar part of the Riemann curvature, $S_{abcd}$, is smooth.

For the same reason, the Kulkarni-Nomizu product between the metric tensor and the term $a^{-2}(t)\beta(t) g_{ab}$ from the expression of the Ricci curvature \eqref{eq_flrw_curv_ricci_a} is smooth.

The only term from \eqref{eq_flrw_curv_ricci_a} we have to check that is smoothened by the Kulkarni-Nomizu product with $g$ is $a^{-2}(t)u_a u_b$. Since $u_a=g_{as}u^s$ and $g$ is diagonal, it follows that $u_a=g_{aa}u^a$ (without summation). If $b\neq t$ ($a\neq t$  is similar), then $u_b=g_{bb}u^b$ contains the needed $a^2(t)$. In the case when $a=b=t$, $a^{-2}(t) u_t u_t$ is not necessarily smooth, but in the Kulkarni-Nomizu product it will appear only in terms of the form $a^{-2}(t) u_t u_t g_{cc}$, with $c\neq t$. Hence, $\Ric\circ g$ is smooth. From this and from the smoothness of $S_{abcd}$, it follows that $E_{abcd}$ is also smooth.

One of the properties of the {\FLRW} metric is that it is conformally flat, that is, $C_{abcd} = 0$. From this it follows that $R_{abcd}=S_{abcd}+E_{abcd}$ is smooth too.
\end{proof}





%--------------------------------------------------------
\subsection{Properties of the proposed equation}
\label{s_properties}


%--------------------------------------------------------
\subsubsection{The Bianchi identity}

We will show that the Riemann curvature tensor satisfies the Bianchi identity
\begin{equation}
	R_{(abc)d;e} = 0.
\end{equation}
Given that it holds at all the points for which $a(t)\neq 0$, where the metric is regular, it also holds by continuity at $a(t)= 0$. But we need to check that the covariant derivatives $(\Ric\circ g)_{abcd;e}$ are smooth, because if the Bianchi identity would be between infinte values, there would be no continuity.

Since the Weyl part of the Riemann curvature $C_{abcd}=0$ in the {\FLRW} spacetime, and from the equations \eqref{eq_flrw_curv_ricci_a} and \eqref{eq_flrw_curv_scalar_a}, it follows that $R_{abcd}$ has the following form:
\begin{equation}
	R_{abcd} = a^{-2}(t)\mu(t) \((u\otimes u)\circ g\)_{abcd} + a^{-2}(t)\nu(t) (g\circ g)_{abcd},
\end{equation}
where the functions $\mu(t)$ and $\nu(t)$ are smooth.

Let's denote by $h_{ij}$, $1\leq i,j\leq 3$, the metric on $\Sigma$. Then $g_{ij}=a^2(t)h_{ij}$. Given that our frame is comoving with the fluid, $u_t=1$, and $u_i=0$ for all $i$. The only terms $a^{-2}(t)\mu(t) \((u\otimes u)\circ g\)_{abcd}$ which don't vanish by containing $u_i=0$ are of the form $a^{-2}(t)\mu(t)u_tu_tg_{ii}$. The covariant derivatives with respect to $t$ cancel one another in the Bianchi identity under the permutation, because the index $t$ is repeated. So we check now those terms of the form $\nabla_j\(a^{-2}(t)\mu(t)u_tu_tg_{ii}\)$, where $i\neq j$. But $\nabla_j\(a^{-2}(t)\mu(t)u_tu_tg_{ii}\)=a^{-2}(t)\mu(t)u_tu_tg_{ii;j}=0$, because only $g_{ii}$ depends on the spacelike direction $x^j$, and because the metric tensor is parallel \eqref{eq_parallel_metric}.

The terms $a^{-2}(t)\nu(t) (g\circ g)_{abcd}$ can only be of the form $a^{-2}(t)\nu(t) g_{aa}g_{bb}$, $a\neq b$. Since $\nabla_i\(a^{-2}(t)\nu(t) g_{aa}g_{bb}\) = a^{-2}(t)\nu(t) \(g_{aa;i}g_{bb} + g_{aa}g_{bb;i}\) = 0$, it follows that the covariant derivatives with respect to $i$ vanish. We check now thosw with respect to $t$. If either the index $a$ or $b$ is equal to $t$, then the cyclic permutation involved in the Bianchi identity vanishes. Then the only remaining possibility is $\nabla_t\(a^{-2}(t)\nu(t) g_{ii}g_{jj}\)$. But $\nabla_t\(a^{-2}(t)\nu(t) g_{ii}g_{jj}\) = -2\dot a(t)a^{-3}(t)\nu(t) g_{ii}g_{jj} + a^{-2}(t)\dot\nu(t) g_{ii}g_{jj}= -2\dot a(t)a(t)\nu(t) h_{ii}h_{jj} + a^{2}(t)\dot\nu(t) h_{ii}h_{jj}$, which is smooth.

Hence, the Bianchi identity makes sense even at the singularity $a(t)=0$.


==> sections/bh-info.tex <==
\section{Information loss}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
\subsection{The significance of the {\semireg} solution}
\label{s_schw_semireg_significance}

The main consequence of the extensibility of the {\schw} solution to a {\semireg} solution beyond the singularity is that the information is not lost there. This can apply as well to the case of an evaporating black hole (see Fig. \ref{evaporating-bh-s}).

Because of the no-hair theorem, the {\schw} solution is representative for non-rotating and electrically neutral black holes. If the black hole evaporates, the information reaching the singularity is lost (Fig. \ref{evaporating-bh-s} A). If the singularity is {\semireg}, it doesn't destroy the topology of spacetime (Fig. \ref{evaporating-bh-s} B). Moreover, although normally in this case the covariant derivative and other differential operators can't be defined, there is a way to construct them naturally (as shown in \cite{Sto11a}), allowing the rewriting of the field equations for the {\semireg} case, without running into infinities. This ensures that the field equations can go beyond the singularity.

\image{evaporating-bh-s}{0.7}{The Penrose-Carter diagram for a non-rotating and electrically neutral evaporating black hole, whose singularity destroys the information.
\textbf{A.} Standard evaporating black hole.
\textbf{B.} Evaporating black hole extended beyond the singularity, whose singularity doesn't destroy the information.}

In the case of a black hole which is not primordial and evaporates completely in a finite time, all of the light rays traversing the singularity reach the past and future infinities. This means that the presence of a spacelike evaporating black hole is compatible with the global hyperbolicity, as in the diagram \ref{evaporating-bh-s} B.

The singularity is accompanied by violent and very destructive forces. But, as we can see from the {\semireg} formulation, there is no reason to consider that it destroys the information or the structure of spacetime.


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
\subsection{The meaning of the analytic extension at the singularity}
\label{s_rn_analytic_meaning}

As in the case of the extension of the {\schw} solution, we can see that the singularity is not necessarily harmful for the information or the structure of spacetime. There is no reason to believe that the information is lost at the singularity, and the fact that it is timelike and may be naked, although it contradicts Penrose's cosmic censorship hypothesis, is compatible with the global hyperbolicity. These observations may apply also to the case of an evaporating charged black hole (see figure \ref{diamond-t}).

The {\rn} solution is, according to the no-hair theorem, representative of non-rotating and electrically charged black holes. If the black hole evaporates, the singularity becomes visible to the distant observers. This is a problem in the solutions which do not admit extension through the singularity. Our solution, because it can be extended beyond the singularity, does not break the topology of spacetime. The metric tensor does not run into infinities, although, because of its degeneracy, other quantities, such as its inverse, may become infinite.

The maximal globally hyperbolic extensions from section \sref{s_rn_globally_hyperbolic} are ideal, because the {\rn} solutions describe spacetimes which are too simple. But because they can be foliated by Cauchy hypersurfaces, and the base hypersurface is $\R^3$, we can interpolate between such solutions and foliations without singularities, and construct more general solutions. The interpolation can be done by varying the parameters $m$ and $q$. By this, one can model spacetimes with black holes that are formed and then evaporate. The presence of a timelike evaporating singularity of this type is compatible with the global hyperbolicity, as in figure \ref{diamond-t}.

\image{diamond-t}{0.5}{Non-primordial evaporating black hole with timelike singularity. The fact that the points of the singularity become visible to distant observers is not a problem for the global hyperbolicity, because the null geodesics can be extended beyond the singularity.}

This extension of the {\rn} solution can be used to model electrically charged particles as charged black holes, as pointed out in Remark \ref{rem_rn_wormhole}.


==> sections/open-problems.tex <==


\begin{openproblem}
What can we say about the other stationary black hole solutions?
In \cite{Sto11f} and \cite{Sto11g} we showed that there are coordinate transformations which make the {\rn} metric and the {\kn} metric analytic at the singularity. This is already a big step, because it allows us to foliate with Cauchy hypersurfaces these spacetimes. Is it possible to find coordinate transformations which make them {\quasireg} too?
\end{openproblem}


\subsection{Open Question}

We conclude with the following open question:
\begin{openproblem}
Are {\quasireg} spacetimes general enough to cover all possible singularities of General Relativity?
\end{openproblem}


\begin{openproblem}
Can we find natural conditions ensuring the uniqueness of the analytic extensions of the {\schw} solution at the singularity $\tau=0$? Or can we consider all analytic extensions of this type to be equivalent, via coordinate changes which may be singular?
\end{openproblem}


To support the second possibility, we can make the observation that the Jacobian from the Remark \ref{rem_jacobian} is degenerate when we pass from a coordinate system characterized by $T=2$ to another one with another value of $T$, but the converse is not true.


A \textit{\semireg} metric has smooth Riemann curvature $R_{abcd}$, and allows the construction of more useful operations which are normally prohibited by the fact that the metric is degenerate. In the case of the {\schw} black hole we could find a solution which is {\semireg} \cite{Sto11e}. In the case of the {\rn} black hole, we can't find numbers $S$ and $T$ for the equation \eqref{eq_coordinate_ext_ext}, which would make the metric \semireg. However, this does not exclude other changes of the coordinates, and we propose the following open problem:
\begin{openproblem}
Is it possible to find coordinates which allow the {\rn} metric to be {\semireg} at $\rho=0$?
\end{openproblem}
Also, it may be interesting the following:
\begin{openproblem}
Can we find natural conditions ensuring the uniqueness of the analytic extensions of the {\schw} and {\rn} solutions at the singularity $\rho=0$? Under what conditions does a singular coordinate transformation of an analytic extension lead to another extension which is physically indistinguishable?
\end{openproblem}


One of the major problems of electrodynamics is the fact that the gauge potential and field become infinite as approaching $r=0$. This problem turns out to be removed, by employing our non-singular coordinate system. This sets as one priority in the future developments of our program to see exactly what happens in the perturbative expansions and in the renormalization group analysis.

